Visual Cross-View Metric Localization with Dense Uncertainty Estimates

This work addresses visual cross-view metric localization for outdoor robotics. Given a ground-level color image and a satellite patch that contains the local surroundings, the task is to identify the location of the ground camera within the satellite patch. Related work addressed this task for range-sensors (LiDAR, Radar), but for vision, only as a secondary regression step after an initial cross-view image retrieval step. Since the local satellite patch could also be retrieved through any rough localization prior (e.g. from GPS/GNSS, temporal filtering), we drop the image retrieval objective and focus on the metric localization only. We devise a novel network architecture with denser satellite descriptors, similarity matching at the bottleneck (rather than at the output as in image retrieval), and a dense spatial distribution as output to capture multi-modal localization ambiguities. We compare against a state-of-the-art regression baseline that uses global image descriptors. Quantitative and qualitative experimental results on the recently proposed VIGOR and the Oxford RobotCar datasets validate our design. The produced probabilities are correlated with localization accuracy, and can even be used to roughly estimate the ground camera's heading when its orientation is unknown. Overall, our method reduces the median metric localization error by 51%, 37%, and 28% compared to the state-of-the-art when generalizing respectively in the same area, across areas, and across time.

==> 5-limitations.tex <==
\section{Limitations and potential social impact}
\label{sec:limitations}
Currently, our single-frame error is still too large for autonomous driving tasks which require sub-meter accuracy.
%The model also does not yet generalize well to new areas.
The multi-modal output also increases the risk of large errors if the wrong mode is selected, compared to (uni-modal) regression.
It remains unclear how more training data will affect the quality, or how robust the model is against outdated satellite imagery.
% Beside, our method is based on the assumption that the known satellite patch is correct and "the car heading is known. 
Finally,
for applications that \textit{do} require global localization, our model does not provide a global satellite descriptor for retrieval as CVR does.

A potential privacy risk in cross-view visual localization is that a personal outdoor photo may unintentionally leak someone's whereabouts.
Still, in this respect global localization (e.g. through image retrieval) poses a larger threat, since our method requires that the approximate location is already known.
Finally, more ground-level data collection to increase the target area implies that more imagery of the public space must be collected, which needs to be properly anonymized and safely stored.

